A PyTorch Library for Hyperspectral Image Models: Technical Report

Hyperspectral remote sensing has advanced across diverse deep learning paradigms, including spectral spatial CNNs, Vision Transformers, Mamba, graph neural networks, Kolmogorov Arnold networks, and self supervised masked autoencoding. Yet progress remains hindered by fragmented repositories, incompatible tensor conventions, and non standardized evaluation. Hyperspectral Image Models addresses these challenges through a modular framework unifying 55 representative models across six paradigms with a common registry, automatic 4D/5D tensor adaptation, and standardized constructors. It integrates 24 benchmark scenes from Airborne, Spaceborne, UAV, and Mars CRISM sensors, with caching, label remapping, PCA, explicit band selection or raw spectra, optional spatial max pooling, and arbitrary PxP patch extraction. To prevent inflated accuracy from overlapping windows, it supports class balanced random partitioning and spatially disjoint regional blocking with Chebyshev guard bands that eliminate train test pixel overlap. Experiments use a single config with deterministic seeds and complete provenance, generating LaTeX benchmark tables and classification maps. Across 1,320 model scene evaluations and 6,600 seeded runs, scene difficulty dominates architecture, with mean accuracy ranging from 96.40% on Botswana to 56.70% on Houston 2018, versus a 15 point spread across paradigm means. No paradigm universally dominates, while sub 1 M parameter models can match architectures two orders of magnitude larger. Code is publicly available at https://github.com/Tanishq251/Hyperspectral-Image-Models.

==> table/complexity.tex <==
%% generated by figures_src/make_tables.py -- do not edit by hand
%% source: Instructions_HSI_Pipeline_arXiv.md section 9 (extracted from models/registry.py and config/dataset.yaml)
\begin{table}[p]
\centering
\caption{Trainable parameters and multiply-accumulate operations for every
implemented architecture, produced by \texttt{model\_info.py} under one fixed probe
input of shape $(1,1,30,11,11)$ at 16 classes. Both are structural properties of the
architecture measured under identical conditions; neither is a performance
measurement, and neither implies any ordering of quality. $^{\dagger}$~probed at
$8\times8$, the smallest patch size satisfying GSCViT's divisibility constraint
(\Cref{sec:repro}). A dash marks a model whose operation count the profiler
could not resolve.}
\label{tab:complexity}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{minipage}[t]{0.485\linewidth}
\centering
\begin{tabular}{@{}lrrr@{}}
\toprule
Model & Params (M) & MACs (M) & Patch \\
\midrule
\multicolumn{4}{@{}l}{\textit{CNN}} \\[1pt]
\quad \texttt{DBDA} & 0.113 & 47.29 & 11 \\
\quad \texttt{DKDMN} & 1.344 & 101.52 & 11 \\
\quad \texttt{ENL\_FCN} & 0.089 & 11.18 & 11 \\
\quad \texttt{FETNet} & 0.492 & -- & 11 \\
\quad \texttt{HybridSN} & 0.535 & 16.01 & 11 \\
\quad \texttt{pResNet} & 0.510 & 15.87 & 11 \\
\quad \texttt{S3ANet} & 0.197 & 10.21 & 11 \\
\quad \texttt{SACNet} & 0.108 & 7.98 & 11 \\
\quad \texttt{SSRN} & 0.136 & 42.00 & 11 \\
\quad \texttt{SSTN} & 0.012 & 1.66 & 11 \\
\addlinespace
\multicolumn{4}{@{}l}{\textit{Transformer}} \\[1pt]
\quad \texttt{3DConvSST} & 0.358 & 79.42 & 11 \\
\quad \texttt{CTMixer} & 0.619 & 73.28 & 11 \\
\quad \texttt{DBCTNet} & 0.003 & 1.78 & 11 \\
\quad \texttt{DSFormer} & 0.677 & 21.05 & 11 \\
\quad \texttt{FAHM} & 0.685 & 11.01 & 11 \\
\quad \texttt{GAHT} & 1.058 & 127.87 & 11 \\
\quad \texttt{GSCViT}$^{\dagger}$ & 0.134 & 3.77 & 8 \\
\quad \texttt{HSIC\_SClusterFormer} & 1.961 & 194.10 & 11 \\
\quad \texttt{MASSFormer} & 0.311 & 15.44 & 11 \\
\quad \texttt{MFT} & 0.629 & 8.09 & 11 \\
\quad \texttt{MMFormer} & 4.436 & 615.13 & 11 \\
\quad \texttt{MorphFormer} & 0.142 & 5.23 & 11 \\
\quad \texttt{MVAHN} & 0.385 & 19.39 & 11 \\
\quad \texttt{S2Gformer} & 0.192 & 11.23 & 11 \\
\quad \texttt{SpectralFormer} & 0.121 & 3.84 & 11 \\
\quad \texttt{SSFTTNet} & 0.153 & 6.99 & 11 \\
\bottomrule
\end{tabular}
\end{minipage}\hfill
\begin{minipage}[t]{0.485\linewidth}
\centering
\begin{tabular}{@{}lrrr@{}}
\toprule
Model & Params (M) & MACs (M) & Patch \\
\midrule
\multicolumn{4}{@{}l}{\textit{Mamba / SSM}} \\[1pt]
\quad \texttt{ConvVitMamba} & 0.523 & 184.73 & 11 \\
\quad \texttt{EMamba} & 0.092 & 4.85 & 11 \\
\quad \texttt{FuzzySpectralMamba} & 4.255 & 345.04 & 11 \\
\quad \texttt{GraphMamba} & 0.703 & 17.55 & 11 \\
\quad \texttt{HyperMamba} & 0.162 & 2.66 & 11 \\
\quad \texttt{HyPyraMamba} & 0.782 & 20.82 & 11 \\
\quad \texttt{IGroupSS-Mamba} & 0.135 & 6.30 & 11 \\
\quad \texttt{MambaHSI} & 0.121 & 0.24 & 11 \\
\quad \texttt{MambaHSI\_Plus} & 0.461 & 0.44 & 11 \\
\quad \texttt{MambaLG} & 0.182 & 14.86 & 11 \\
\quad \texttt{MambaMoE} & 0.897 & 9.77 & 11 \\
\quad \texttt{MHSSMamba} & 0.052 & 4.94 & 11 \\
\quad \texttt{MiM} & 0.074 & 49.70 & 11 \\
\quad \texttt{MLFMamba} & 0.260 & 16.05 & 11 \\
\quad \texttt{MorpMamba} & 0.071 & 5.78 & 11 \\
\quad \texttt{PHDMamba} & 0.362 & 13.97 & 11 \\
\quad \texttt{R2Mamba} & 0.420 & 3.29 & 11 \\
\quad \texttt{S2Mamba} & 0.116 & 8.73 & 11 \\
\quad \texttt{SSMamba} & 1.035 & 37.75 & 11 \\
\quad \texttt{WaveMamba} & 0.080 & 6.44 & 11 \\
\addlinespace
\multicolumn{4}{@{}l}{\textit{Graph / GCN}} \\[1pt]
\quad \texttt{GraphGST} & 0.022 & 1.94 & 11 \\
\quad \texttt{GTCFN} & 0.250 & 28.04 & 11 \\
\quad \texttt{MCTGCL} & 0.327 & 26.11 & 11 \\
\quad \texttt{MS2GCAN} & 0.022 & 0.00 & 11 \\
\addlinespace
\multicolumn{4}{@{}l}{\textit{KAN}} \\[1pt]
\quad \texttt{HSIConvKAN} & 0.434 & 1.23 & 11 \\
\quad \texttt{HyperKAN} & 0.344 & 11.11 & 11 \\
\addlinespace
\multicolumn{4}{@{}l}{\textit{Self-supervised}} \\[1pt]
\quad \texttt{HSIC\_FM} & 34.229 & 4195.03 & 11 \\
\quad \texttt{HSIMAE} & 3.616 & 229.48 & 11 \\
\quad \texttt{LFSMIM} & 0.513 & 16.28 & 11 \\
\bottomrule
\end{tabular}
\end{minipage}
\end{table}


==> table/datasets.tex <==
%% generated by figures_src/make_tables.py -- do not edit by hand
%% source: Instructions_HSI_Pipeline_arXiv.md section 9 (extracted from models/registry.py and config/dataset.yaml)
\begin{table}[t]
\centering
\caption{The 24 scenes the framework distributes and loads. Dimensions, band
counts, class counts and labelled-pixel counts are read from
\texttt{config/dataset.yaml}; sensors, platforms and regions are recorded in
\texttt{docs/DATASETS.md}. Labelled pixels exclude the unlabelled background
class, which the loader drops. The count spans roughly two and a half orders of
magnitude, from Botswana to Pingan, which is a practical constraint on memory,
runtime and sensible split sizes rather than a property of any architecture. Scene
names here are the published ones; Tangdaowan is registered in
\texttt{config/dataset.yaml} under the key \texttt{Tangdoaowan}, which is the
string a configuration file must use.}
\label{tab:datasets}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrll@{}}
\toprule
Scene & Size ($H\times W$) & Bands & Classes & Labelled px & Sensor (platform) & Region \\
\midrule
Augsburg & 332$\times$485 & 180 & 7 & 78,294 & DAS Specim (airborne) & Augsburg, Germany \\
Berlin & 1723$\times$476 & 244 & 8 & 464,671 & HyMap (airborne) & Berlin, Germany \\
Botswana & 1476$\times$256 & 145 & 14 & 3,248 & EO-1 Hyperion (spaceborne) & Okavango Delta, Botswana \\
Chikusei & 2517$\times$2335 & 128 & 19 & 77,592 & Headwall Photonics (airborne) & Chikusei, Japan \\
Dioni & 250$\times$1376 & 176 & 12 & 20,024 & AVIRIS-NG (airborne) & Dioni, Greece \\
Holden & 595$\times$440 & 418 & 6 & 20,090 & MRO CRISM (orbital) & Mars \\
Houston13 & 349$\times$1905 & 144 & 15 & 15,029 & ITRES CASI-1500 (airborne) & Houston, TX, USA \\
Houston18 & 1202$\times$4768 & 48 & 20 & 15,029 & AVIRIS-NG (airborne) & Houston, TX, USA \\
Indian\_Pines & 200$\times$145 & 145 & 16 & 10,249 & AVIRIS (airborne) & Indiana, USA \\
KSC & 512$\times$614 & 176 & 13 & 5,211 & AVIRIS (airborne) & Florida, USA \\
Loukia & 249$\times$945 & 176 & 14 & 13,503 & AVIRIS-NG (airborne) & Loukia, Greece \\
Muufl & 325$\times$220 & 64 & 11 & 53,687 & ITRES CASI-1500 (airborne) & Mississippi, USA \\
NiliFossae & 478$\times$593 & 425 & 9 & 26,710 & MRO CRISM (orbital) & Mars \\
Pavia Center & 1096$\times$715 & 102 & 9 & 148,152 & ROSIS (airborne) & Pavia, Italy \\
Pavia University & 610$\times$340 & 103 & 9 & 42,776 & ROSIS (airborne) & Pavia, Italy \\
Pingan & 1230$\times$1000 & 176 & 10 & 1,140,937 & Gaiasky mini2-VNIR (uav) & Qingdao, China \\
Qingyun & 880$\times$1360 & 176 & 6 & 954,893 & Gaiasky mini2-VNIR (uav) & Qingdao, China \\
Salinas & 512$\times$217 & 204 & 16 & 54,129 & AVIRIS (airborne) & Salinas Valley, USA \\
Tangdaowan & 1740$\times$860 & 176 & 18 & 557,366 & Gaiasky mini2-VNIR (uav) & Qingdao, China \\
Trento & 166$\times$600 & 63 & 6 & 30,214 & AISA Eagle (airborne) & Trento, Italy \\
Utopia & 478$\times$595 & 432 & 9 & 17,338 & MRO CRISM (orbital) & Mars \\
WHU-Hi-HanChuan & 1217$\times$303 & 274 & 16 & 257,530 & Headwall Nano (uav) & HanChuan, China \\
WHU-Hi-HongHu & 940$\times$475 & 270 & 22 & 386,693 & Headwall Nano (uav) & HongHu, China \\
WHU-Hi-LongKou & 550$\times$400 & 270 & 9 & 204,542 & Headwall Nano (uav) & LongKou, China \\
\bottomrule
\end{tabular}
\end{table}


==> table/deviations.tex <==
%% generated by figures_src/make_appendix_tables.py -- do not edit by hand
\begin{table}[p]
\centering
\caption{Documented deviations from the authors' released code, extracted
automatically from the module docstring at the head of each model file.
\texttt{docs/CONTRIBUTING.md} makes such a note a condition of adding a model, so
every adaptation stays traceable to the original work; models absent from this
table required no documented change. The wording is the repository's, lightly
condensed.}
\label{tab:deviations}
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}>{\raggedright}p{0.16\linewidth}p{0.80\linewidth}@{}}
\toprule
Model & Documented deviation \\
\midrule
\multicolumn{2}{@{}l}{\textit{CNN}} \\[1pt]
\texttt{DKDMN} & Adapted to the unified library API:; Helper modules (ChebConv / CNN\_ViT / embeddings) moved under models/helpers/dkdmn\_; and imports rewired accordingly.; The trailing demo block and module-level `device = torch.device(...)` were dropped.; The reference MultiViewNet returns (features, logits) with the batch doubled, because it concatenates its two views. `DKDMNClassifier` below averages the two views' logits so the model exposes the standard (B, num\_classes) contract the trainer expects.; `datasetname` is left empty so the generic `else` branches are used (groups=11, groups\_width=37, emb/head/hidden dims 256/128/128). \\
\addlinespace[2pt]
\texttt{ENL\_FCN} & This implementation adapts the ENL-FCN model to the unified API. The original model uses Criss-Cross Attention for efficient non-local feature extraction. \\
\addlinespace[2pt]
\texttt{HybridSN} & Adapted from Pancakerr/HybridSN --- uses dummy forward pass at init to dynamically compute intermediate feature dimensions instead of lazy init. \\
\addlinespace[2pt]
\texttt{pResNet} & Adapted to the unified library API. Changes vs. the original reference code:; The shortcut AvgPool2d now uses ceil\_mode=True. The original floors the spatial size (11 -> 5) while the stride-2 conv ceils it (11 -> 6), which crashes on odd patch sizes such as 11.; The zero-padding tensor for channel matching is created on the input's device instead of a hardcoded .cuda().; The final pooling is AdaptiveAvgPool2d(1) so any patch size works without hand-computing `avgpoosize`. \\
\addlinespace[2pt]
\addlinespace[3pt]
\multicolumn{2}{@{}l}{\textit{Transformer}} \\[1pt]
\texttt{DSFormer} & Adapted from original repo to work with local model registry. \\
\addlinespace[2pt]
\texttt{GSCViT} & Deviations from the authors' released code:; Fixed an einops axis name in the ``num\_groups == 1`` branch of ``GSSA.forward`` (``g=gss`` -> ``g1=gss``). That branch raises in the original and is unreachable behind its assert, so this is a latent-bug fix, not a behavioural change.; Added ``@register\_model`` plumbing and standardised the ``bands`` -> ``channels`` keyword so the model matches the pipeline's common interface. \\
\addlinespace[2pt]
\texttt{MVAHN} & Adapted to the unified library API:; Helper modules (ChebConv / Transformer / Embeddings) moved under models/helpers/mvahn\_; and imports rewired accordingly.; The unused `datasetname` constructor argument is defaulted.; `np.squeeze(x, axis=1)` replaced with a native `x.squeeze(1)`.; The original \_\_main\_\_ demo block and torchsummary import were dropped. \\
\addlinespace[2pt]
\addlinespace[3pt]
\multicolumn{2}{@{}l}{\textit{Mamba / SSM}} \\[1pt]
\texttt{ConvVitMamba} & Adaptation notes:; Original implementation is TensorFlow/Keras (functional API). Ported to PyTorch layer-for-layer, preserving the same pipeline: a multi-scale 3D conv front-end (MS\_FE: spectral-only, spatial-only, and joint spectral-spatial 3D conv branches over the raw HSI cube) -> non-overlapping patch tokenization -> a 4-layer standard ViT transformer encoder -> an MLP head -> a gated-convolution "Mamba block" (the repo's own lightweight conv-gated sequence-mixing block, not `mamba\_ssm`) -> global average pool -> classifier.; Keras `layers.MultiHeadAttention(num\_heads, key\_dim=projection\_dim)` uses an internal q/k/v width of `num\_heads*key\_dim` distinct from the input embedding dim, with an output projection back down --- this is reproduced exactly with a small custom attention module (`KerasStyleMHA`) since `nn.MultiheadAttention` assumes embed\_dim is evenly split across heads.; The final Keras `Dense(num\_classes, activation="softmax")` is replaced with raw logits (no softmax) per this framework's convention.; `MS\_FE`'s 3D convs operate on the raw cube (H, W, bands, 1) in Keras' channels-last layout; this is the framework's `expects\_4d=False` 5D input (B, 1, bands, H, W), so `expects\_4d=False` is used here. \\
\addlinespace[2pt]
\texttt{EMamba} & Adaptation notes:; E-Mamba is originally an HSI+LiDAR fusion model: the original `MultimodalClassier.forward(x1, x2)` runs an HSI cube (x1) and a LiDAR cube (x2, projected to the same channel count) through four *shared; VSSBlock stacks and then fuses them with a cross-Mamba attention block + a concat-Mamba fusion block, before a linear classifier head.; This benchmark provides only single-modality HSI input, so the LiDAR branch (`conv\_lidar`) and both fusion blocks (`CrossMambaFusionBlock`, `ConcatMambaFusionBlock`) are dropped. What remains is exactly the HSI stream of the original model --- the same four VSSBlocks applied to x1 in sequence --- followed by the same average-pool classifier + linear head. No new layers are introduced; only the parts that require a second modality are removed.; The custom CUDA kernel `selective\_scan\_cuda\_core` (bundled with this repo's own build, not the pip `mamba\_ssm` package) is unavailable here. It is replaced with the algebraically equivalent pure-PyTorch reference scan `mamba\_ssm.ops.selective\_scan\_interface.selective\_scan\_ref`, used exactly as the VMamba-style `forward\_corev2` selective-scan needs it. \\
\addlinespace[2pt]
\texttt{GraphMamba} & Adapted to the unified HSI classification framework:; Removed hard-coded .cuda() calls \$\textbackslash\{\}rightarrow\$ device-agnostic; forward() accepts standard 5D input and returns only logits; Adjacency matrix computed internally from patch data; All hyper-parameters exposed via register\_model() defaults \\
\addlinespace[2pt]
\texttt{HyperMamba} & Adaptation notes:; The original repo builds on a VMamba (VSSM) backbone with two custom CUDA kernels (selective\_scan\_cuda\_core / selective\_scan\_cuda\_oflex) compiled as part of the VMamba project itself (not the pip `mamba\_ssm` package, and not available in this environment). These are replaced here with the algebraically-equivalent pure-PyTorch reference scan (`mamba\_ssm.ops.selective\_scan\_interface.selective\_scan\_ref`), which supports the same grouped B/C broadcasting the kernels used. This is a drop-in numerical substitute, not an architectural change.; The model also uses `mmcv.ops.DeformRoIPool` for a 4-scale RoI pooling + Gumbel-softmax routing front-end. mmcv (compiled ops) is not installed in this environment. Because the original code calls DeformRoIPool with no offset tensor, it degenerates to standard box RoI pooling, so it is replaced with `torchvision.ops.roi\_align` over the same boxes --- same operation, no mmcv dependency.; Triton cross-scan kernels, fvcore FLOP counters, and openmmlab backbone-compat wrappers (unused at inference) were dropped as dead code. \\
\addlinespace[2pt]
\texttt{MambaLG} & Adapted from the authors' PyTorch implementation (mambaLG.py). Kept the architecture (multi-scale spatial conv fusion -> local windowed Mamba -> global Mamba over the whole spatial token sequence -> spectral-band-group Mamba -> spatial x spectral gating -> classification head) faithful; the authors' `Mamba` block (mamba\_simple.py, a local copy of mamba\_ssm's Mamba) is replaced with `mamba\_ssm.Mamba` directly (same architecture, already a framework dependency). Hardcoded `.cuda()`/`self.device` calls in the original `forward` were replaced with device-agnostic tensor ops so the model runs on CPU or GPU. `spa\_token` is exposed as a constructor kwarg (the authors hardcode 12 in their `main.py`). \\
\addlinespace[2pt]
\texttt{MHSSMamba} & Note: the original repo ships only a Colab notebook (MHSSMamba\_Git.ipynb) with a TensorFlow/Keras model (`SSMambaModel`, built from `SpectralSpatialTokenGeneration`, `MultiHeadAttention`, `SpectralSpatialFeatureEnhancement` and a recurrent `StateSpaceModel`). This file is a faithful PyTorch port of that architecture: spectral/spatial linear tokenization -> multi-head cross attention between the two token streams -> center-token gated feature enhancement -> a simple recurrent state-space aggregator -> linear classifier. A couple of shape bugs in the original notebook (e.g. indexing/broadcasting that only worked for the specific demo tensor shapes) were fixed so the module works for arbitrary patch sizes/band counts while preserving the intended data flow. \\
\addlinespace[2pt]
\texttt{MorpMamba} & Note: the original repo ships only a Colab notebook ("Spatial-Spectral MorpMamba.ipynb") implemented in TensorFlow/Keras. This file is a faithful PyTorch port of that architecture: learnable morphological erosion/dilation "tokenization" (depthwise box-filter convs initialized to an all-ones structuring element, as in the original `ErosionLayer`/ `DilationLayer`) producing spatial and spectral token maps -> multi-head cross attention between the two streams -> center-token gated feature enhancement -> a simple recurrent state-space aggregator -> MLP classifier. A couple of shape bugs in the original notebook (indexing/broadcasting that only worked for the specific demo tensor shapes) were fixed so the module works for arbitrary patch sizes/band counts while preserving the intended data flow. \\
\addlinespace[2pt]
\texttt{WaveMamba} & Original implementation in TensorFlow/Keras. This is a faithful PyTorch port adapted to work with the local model registry. \\
\addlinespace[2pt]
\addlinespace[3pt]
\multicolumn{2}{@{}l}{\textit{KAN}} \\[1pt]
\texttt{HSIConvKAN} & Adapted here for the framework's variable bands/patch\_size interface:; effConvKAN3D originally depends on the external `unfoldNd` package; that unfold is reimplemented inline below with plain `torch.Tensor.unfold` (no extra dependency), producing identical patches.; The reference notebook hardcodes a maxpool kernel/final KAN input width (`nn.MaxPool2d(kernel\_size=3, stride=3)` then `KAN([64, 32, NUM\_CLASS])`) that only happens to work for its own patch\_size and breaks for others (pooling a height-1 feature map with a kernel of 3). We keep the same layer stack (3x effConvKAN3D -> ConvKAN2D -> KAN head) but swap the fixed maxpool for `nn.AdaptiveMaxPool2d`, which reproduces the same kind of downsampling while making the classifier head's input size (and thus the whole model) independent of `patch\_size`/`bands`.; KAN layer implementations (KANLinear / Fast\_KANLinear / FastKAN) are bundled inline from HSIConvKAN/kan\_linear.py and HSIConvKAN/fast\_kan.py (both pure PyTorch, no extra dependency; fast\_kan.py itself is a copy of https://github.com/ZiyaoLi/fast-kan bundled in the original repo). \\
\addlinespace[2pt]
\texttt{HyperKAN} & Adapted from f-neumann77/HyperKAN --- models/ssftt\_full\_kan.py and models/kan\_layers.py (KAN layer implementations bundled inline below, based on https://github.com/IvanDrokin/torch-conv-kan, itself derived from https://github.com/Blealtan/efficient-kan; no extra pip dependency needed). The original n\_bands-dependent conv2d input width is now computed dynamically instead of assuming a hardcoded band count, so the model works for any `bands`/`patch\_size` the framework passes in. \\
\addlinespace[2pt]
\bottomrule
\end{tabular}
\end{table}


==> table/models.tex <==
%% generated by figures_src/make_tables.py -- do not edit by hand
%% source: Instructions_HSI_Pipeline_arXiv.md section 9 (extracted from models/registry.py and config/dataset.yaml)
\begin{table}[p]
\centering
\caption{Every architecture implemented in the framework, grouped by family and
ordered by publication year, with the venue and identifier of the original paper.
Architectural credit for every entry belongs to its original authors; the framework
claims the integration, not the architectures.}
\label{tab:models}
\fontsize{7.8pt}{8.8pt}\selectfont
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}lll l@{}}
\toprule
Model & Year & Venue & Paper \\
\midrule
\multicolumn{4}{l}{\textit{CNN} (11 implemented)} \\[1pt]
\quad \texttt{SSRN} & 2017 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2017.2755542}{10.1109/TGRS.2017.2755542} \\
\quad \texttt{HybridSN} & 2019 & IEEE GRSL & \href{https://doi.org/10.1109/LGRS.2019.2918719}{10.1109/LGRS.2019.2918719} \\
\quad \texttt{pResNet} & 2019 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2018.2860125}{10.1109/TGRS.2018.2860125} \\
\quad \texttt{DBDA} & 2020 & MDPI Remote Sensing & \href{https://doi.org/10.3390/rs12030582}{10.3390/rs12030582} \\
\quad \texttt{ENL\_FCN} & 2020 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2020.3014286}{10.1109/TGRS.2020.3014286} \\
\quad \texttt{SACNet} & 2021 & IEEE TIP & \href{https://doi.org/10.1109/TIP.2021.3118977}{10.1109/TIP.2021.3118977} \\
\quad \texttt{SSTN} & 2021 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2021.3115699}{10.1109/TGRS.2021.3115699} \\
\quad \texttt{3DRCNet} & 2024 & arXiv & \href{https://arxiv.org/abs/2408.13728}{arXiv:2408.13728} \\
\quad \texttt{DKDMN} & 2024 & Expert Syst. Appl. & \href{https://doi.org/10.1016/j.eswa.2024.123796}{10.1016/j.eswa.2024.123796} \\
\quad \texttt{S3ANet} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2024.3381824}{10.1109/TGRS.2024.3381824} \\
\quad \texttt{FETNet} & 2026 & Eng. Appl. Artif. Intell. & \href{https://doi.org/10.1016/j.engappai.2025.113343}{10.1016/j.engappai.2025.113343} \\
\addlinespace
\multicolumn{4}{l}{\textit{Transformer} (16 implemented)} \\[1pt]
\quad \texttt{SpectralFormer} & 2021 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2021.3130716}{10.1109/TGRS.2021.3130716} \\
\quad \texttt{CTMixer} & 2022 & IEEE GRSL & IEEE Xplore 9924229 \\
\quad \texttt{SSFTTNet} & 2022 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2022.3144158}{10.1109/TGRS.2022.3144158} \\
\quad \texttt{GAHT} & 2023 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2022.3207933}{10.1109/TGRS.2022.3207933} \\
\quad \texttt{MFT} & 2023 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2023.3286826}{10.1109/TGRS.2023.3286826} \\
\quad \texttt{MorphFormer} & 2023 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2023.3242346}{10.1109/TGRS.2023.3242346} \\
\quad \texttt{MVAHN} & 2023 & IEEE TGRS & \href{https://doi.org/10.1016/j.eswa.2023.121032}{10.1016/j.eswa.2023.121032} \\
\quad \texttt{3DConvSST} & 2024 & IEEE CAI & \href{https://doi.org/10.1109/CAI59869.2024.00011}{10.1109/CAI59869.2024.00011} \\
\quad \texttt{DBCTNet} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2024.3368141}{10.1109/TGRS.2024.3368141} \\
\quad \texttt{GSCViT} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2024.3377610}{10.1109/TGRS.2024.3377610} \\
\quad \texttt{MASSFormer} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2024.3392264}{10.1109/TGRS.2024.3392264} \\
\quad \texttt{S2Gformer} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2024.3488202}{10.1109/TGRS.2024.3488202} \\
\quad \texttt{DSFormer} & 2025 & Neural Networks & \href{https://doi.org/10.1016/j.neunet.2025.107311}{10.1016/j.neunet.2025.107311} \\
\quad \texttt{FAHM} & 2025 & IEEE JSTARS & \href{https://doi.org/10.1109/JSTARS.2025.3539791}{10.1109/JSTARS.2025.3539791} \\
\quad \texttt{HSIC\_SClusterFormer} & 2025 & IEEE TIP & \href{https://doi.org/10.1109/TIP.2024.3522809}{10.1109/TIP.2024.3522809} \\
\quad \texttt{MMFormer} & 2026 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2026.3696892}{10.1109/TGRS.2026.3696892} \\
\addlinespace
\multicolumn{4}{l}{\textit{Mamba / SSM} (19 implemented)} \\[1pt]
\quad \texttt{GraphMamba} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2024.3493101}{10.1109/TGRS.2024.3493101} \\
\quad \texttt{HyperMamba} & 2024 & IEEE TGRS & IEEE Xplore 10614183 \\
\quad \texttt{IGroupSS-Mamba} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2024.3502055}{10.1109/TGRS.2024.3502055} \\
\quad \texttt{MambaHSI} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2024.3430985}{10.1109/TGRS.2024.3430985} \\
\quad \texttt{MambaHSI\_Plus} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2025.3576656}{10.1109/TGRS.2025.3576656} \\
\quad \texttt{MambaLG} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2024.3521411}{10.1109/TGRS.2024.3521411} \\
\quad \texttt{S2Mamba} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2025.3530993}{10.1109/TGRS.2025.3530993} \\
\quad \texttt{SSMamba} & 2024 & MDPI Remote Sensing & \href{https://doi.org/10.3390/rs16132449}{10.3390/rs16132449} \\
\quad \texttt{WaveMamba} & 2024 & IEEE GRSL & \href{https://doi.org/10.1109/LGRS.2024.3506034}{10.1109/LGRS.2024.3506034} \\
\quad \texttt{ConvVitMamba} & 2025 & Knowledge-Based Syst. & \href{https://doi.org/10.1016/j.knosys.2025.113282}{10.1016/j.knosys.2025.113282} \\
\quad \texttt{MambaMoE} & 2025 & Information Fusion & \href{https://doi.org/10.1016/j.inffus.2025.103811}{10.1016/j.inffus.2025.103811} \\
\quad \texttt{MHSSMamba} & 2025 & Remote Sens. Letters & \href{https://doi.org/10.1080/2150704X.2025.2461330}{10.1080/2150704X.2025.2461330} \\
\quad \texttt{MiM} & 2025 & Neurocomputing & \href{https://doi.org/10.1016/j.neucom.2024.128751}{10.1016/j.neucom.2024.128751} \\
\quad \texttt{MorpMamba} & 2025 & Neurocomputing & \href{https://doi.org/10.1016/j.neucom.2025.129990}{10.1016/j.neucom.2025.129990} \\
\quad \texttt{PHDMamba} & 2025 & IEEE GRSL & \href{https://doi.org/10.1109/LGRS.2025.3626712}{10.1109/LGRS.2025.3626712} \\
\quad \texttt{EMamba} & 2026 & Information Fusion & \href{https://doi.org/10.1016/j.inffus.2025.103328}{10.1016/j.inffus.2025.103328} \\
\quad \texttt{FuzzySpectralMamba} & 2026 & IEEE GRSL & \href{https://doi.org/10.1109/LGRS.2026.3687386}{10.1109/LGRS.2026.3687386} \\
\quad \texttt{HyPyraMamba} & 2026 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2025.3650350}{10.1109/TGRS.2025.3650350} \\
\quad \texttt{MLFMamba} & 2026 & The Visual Computer & \href{https://doi.org/10.1007/s00371-026-04496-w}{10.1007/s00371-026-04496-w} \\
\addlinespace
\multicolumn{4}{l}{\textit{Graph / GCN} (4 implemented)} \\[1pt]
\quad \texttt{GraphGST} & 2024 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2023.3349076}{10.1109/TGRS.2023.3349076} \\
\quad \texttt{GTCFN} & 2025 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2025.3618962}{10.1109/TGRS.2025.3618962} \\
\quad \texttt{MCTGCL} & 2025 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2025.3529996}{10.1109/TGRS.2025.3529996} \\
\quad \texttt{MS2GCAN} & 2026 & IEEE TGRS & \href{https://doi.org/10.1109/TGRS.2026.3678343}{10.1109/TGRS.2026.3678343} \\
\addlinespace
\multicolumn{4}{l}{\textit{KAN} (2 implemented)} \\[1pt]
\quad \texttt{HSIConvKAN} & 2024 & MDPI Remote Sensing & \href{https://doi.org/10.3390/rs16214015}{10.3390/rs16214015} \\
\quad \texttt{HyperKAN} & 2024 & MDPI Sensors & \href{https://doi.org/10.3390/s24237683}{10.3390/s24237683} \\
\addlinespace
\multicolumn{4}{l}{\textit{Self-supervised} (3 implemented)} \\[1pt]
\quad \texttt{HSIC\_FM} & 2024 & IEEE TNNLS & \href{https://doi.org/10.1109/TNNLS.2023.3279377}{10.1109/TNNLS.2023.3279377} \\
\quad \texttt{HSIMAE} & 2024 & arXiv & \href{https://doi.org/10.1109/JSTARS.2024.3432743}{10.1109/JSTARS.2024.3432743} \\
\quad \texttt{LFSMIM} & 2024 & IEEE GRSL & \href{https://doi.org/10.1109/LGRS.2024.3360184}{10.1109/LGRS.2024.3360184} \\
\bottomrule
\end{tabular}
\end{table}


==> table/tab2_architectures.tex <==
\begin{table}[t]
\centering
\caption{Taxonomy of evaluated architectural paradigms, detailing their core mathematical mechanisms, structural inductive biases, and temporal span across the literature.}
\label{tab:paradigms}
\footnotesize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}p{0.14\linewidth}p{0.18\linewidth}cp{0.31\linewidth}p{0.25\linewidth}@{}}
\toprule
Paradigm & Formal Family & Evaluated & Core Mathematical Mechanism & Structural Inductive Bias \\
\midrule
\textbf{CNN} & Convolutional Neural Networks & 10 & Local weight sharing, spatial-spectral 2D/3D convolutions, multi-scale residual kernels & Strong spatial translation invariance, compact parameter footprints \\
\addlinespace[2pt]
\textbf{Transformer} & Vision \& Spectral Transformers & 16 & Multi-head self-attention, spectral/spatial tokenization, cross-attention encoders & Global contextual receptive field, sequence-level spectral dependency modelling \\
\addlinespace[2pt]
\textbf{Mamba / SSM} & State-Space Models (Mamba) & 20 & Continuous-time state-space discretization, selective scan ($S6$), multi-directional scans & Linear-time sequence complexity, long-range dependency tracking without attention quadratics \\
\addlinespace[2pt]
\textbf{Graph / GCN} & Graph Convolutional Networks & 5 & Superpixel adjacency graphs, Chebyshev spectral filtering, topology-aware message passing & Irregular boundary adaptation, non-Euclidean spatial relational inductive bias \\
\addlinespace[2pt]
\textbf{KAN} & Kolmogorov-Arnold Networks & 2 & Learnable univariate B-spline activation functions on network edges, matrix formulation & High non-linear function approximation capacity per parameter, symbolic interpretability \\
\addlinespace[2pt]
\textbf{Self-supervised} & Masked Autoencoders \& FM & 3 & Spectral-spatial masked patch reconstruction, self-supervised pretext representations & Generic spectral representation learning independent of task-specific label supervision \\
\addlinespace[2pt]
\bottomrule
\end{tabular}
\end{table}

==> table/tab3_family_aggregate.tex <==
\begin{table}[t]
\centering
\caption{Aggregate accuracy by paradigm under the protocol of \Cref{tab:protocol}, over all \NumTotalEvaluations{} evaluations. $\sigma$ is the standard deviation over every evaluation in the family and therefore mixes within-model and between-model variation. \emph{Best} counts the scenes on which a member of the family attains the highest accuracy.}
\label{tab:family_aggregate}
\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
Paradigm & Models & Evals & Mean OA & Median OA & $\sigma$ & Mean AA & Mean $\kappa$ & Best \\
\midrule
\textbf{CNN} & 10 & 240 & 86.90 & 89.91 & 11.69 & 88.74 & 83.93 & 7 \\
\textbf{Graph / GCN} & 4 & 96 & 86.72 & 89.31 & 10.88 & 88.53 & 83.65 & 3 \\
\textbf{Mamba / SSM} & 20 & 480 & 84.78 & 89.30 & 15.23 & 86.61 & 81.55 & 8 \\
\textbf{KAN} & 2 & 48 & 84.75 & 86.91 & 12.46 & 87.04 & 81.27 & 0 \\
\textbf{Transformer} & 16 & 384 & 84.33 & 89.73 & 17.38 & 86.36 & 81.24 & 6 \\
\textbf{Self-supervised} & 3 & 72 & 72.02 & 79.75 & 22.83 & 74.79 & 67.13 & 0 \\
\bottomrule
\end{tabular}
\end{table}


==> table/tab5_complexity.tex <==
\begin{table}[t]
\centering
\caption{Representative architectures illustrating the accuracy--complexity trade-off across paradigms, showing trainable parameters, floating-point operations (MACs), mean empirical accuracy, and cross-dataset standard deviation.}
\label{tab:complexity_tradeoffs}
\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{@{}llrrrrr@{}}
\toprule
Model & Paradigm & Year & Parameters (M) & MACs (G) & Mean OA (\%) & Cross-Dataset $\sigma$ \\
\midrule
\texttt{DBDA} & CNN & 2020 & 0.113 & 0.0473 & 90.37 & 9.18 \\
\texttt{3DConvSST} & Transformer & 2024 & 0.358 & 0.0794 & 90.27 & 9.29 \\
\texttt{S2Mamba} & Mamba / SSM & 2024 & 0.116 & 0.0087 & 89.91 & 10.19 \\
\texttt{IGroupSS-Mamba} & Mamba / SSM & 2024 & 0.135 & 0.0063 & 89.87 & 9.78 \\
\texttt{DSFormer} & Transformer & 2025 & 0.677 & 0.0210 & 89.84 & 9.65 \\
\texttt{MambaLG} & Mamba / SSM & 2024 & 0.182 & 0.0149 & 89.82 & 9.73 \\
\texttt{SSFTTNet} & Transformer & 2022 & 0.153 & 0.0070 & 89.62 & 9.81 \\
\texttt{SSRN} & CNN & 2017 & 0.136 & 0.0420 & 89.43 & 10.40 \\
\texttt{MMFormer} & Transformer & 2026 & 4.436 & 0.6151 & 89.28 & 10.15 \\
\texttt{GTCFN} & Graph / GCN & 2025 & 0.250 & 0.0280 & 88.95 & 10.15 \\
\texttt{MS2GCAN} & Graph / GCN & 2026 & 0.022 & < 0.001 & 88.83 & 9.62 \\
\texttt{SpectralFormer} & Transformer & 2021 & 0.121 & 0.0038 & 86.88 & 11.06 \\
\texttt{HyperKAN} & KAN & 2024 & 0.344 & 0.0111 & 86.86 & 11.46 \\
\texttt{SACNet} & CNN & 2021 & 0.108 & 0.0080 & 86.13 & 11.83 \\
\texttt{SSMamba} & Mamba / SSM & 2024 & 1.035 & 0.0377 & 85.26 & 11.94 \\
\texttt{FETNet} & CNN & 2026 & 0.492 & -- & 81.33 & 16.10 \\
\texttt{WaveMamba} & Mamba / SSM & 2024 & 0.080 & 0.0064 & 50.21 & 20.08 \\
\texttt{HSIC\_FM} & Self-supervised & 2024 & 34.229 & 4.1950 & 48.82 & 19.89 \\
\bottomrule
\end{tabular}
\end{table}

==> table/tab6_pending.tex <==
\begin{table}[t]
\centering
\caption{The three implemented architectures whose evaluation was still running when
this version was prepared. They are present in the registry and in \Cref{tab:models},
and are excluded from every aggregate reported in this section. \texttt{GSCViT} is a
separate case: its grouping hierarchy requires a patch size divisible by four
(\Cref{sec:integration}), so it cannot be run at the protocol's $11\times11$ window and
must be reported under a divisible patch size instead.}
\label{tab:pending}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}llcccc@{}}
\toprule
Model & Paradigm & Year & Mean OA (\%) & Mean AA (\%) & Mean $\kappa$ \\
\midrule
\texttt{3DRCNet} \citep{3DRCNet}   & CNN         & 2024 & -- & -- & -- \\
\texttt{DBCTNet} \citep{DBCTNet}   & Transformer & 2024 & -- & -- & -- \\
\texttt{GSCViT}  \citep{GSCViT}    & Transformer & 2024 & -- & -- & -- \\
\bottomrule
\end{tabular}
\end{table}


==> table/tab_class_stats.tex <==
\begin{table}[t]
\centering
\caption{Class structure of every scene and what the shared protocol draws from it. Counts are the per-class sample counts recorded in \texttt{config/dataset.yaml}. The imbalance ratio is the largest class divided by the smallest. Train and validation columns give the fixed budget of 30 and 10 labelled pixels per class; the test column is the remainder, and the final column is the share of the annotation that training consumes, which varies by three orders of magnitude across the collection. Chikusei's per-class breakdown is not recorded in the registry, so its smallest and largest class are left blank.}
\label{tab:classstats}
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
Scene & Cls & Labelled px & Smallest & Largest & Imbal. & Train & Val & Train \% \\
\midrule
Augsburg & 7 & 78,294 & 575 & 30,329 & 53$\times$ & 210 & 70 & 0.27 \\
Berlin & 8 & 464,671 & 6,672 & 268,642 & 40$\times$ & 240 & 80 & 0.05 \\
Botswana & 14 & 3,248 & 95 & 314 & 3$\times$ & 420 & 140 & 12.93 \\
Chikusei & 19 & 77,592 & -- & -- & -- & 570 & 190 & 0.73 \\
Dioni & 12 & 20,024 & 150 & 6,374 & 42$\times$ & 360 & 120 & 1.80 \\
Holden & 6 & 20,090 & 458 & 8,697 & 19$\times$ & 180 & 60 & 0.90 \\
Houston 2013 & 15 & 15,029 & 325 & 1,268 & 4$\times$ & 450 & 150 & 2.99 \\
Houston 2018 & 20 & 2,018,910 & 587 & 894,769 & 1,524$\times$ & 600 & 200 & 0.03 \\
Indian Pines & 16 & 10,249 & 20 & 2,455 & 123$\times$ & 480 & 160 & 4.68 \\
KSC & 13 & 5,211 & 105 & 927 & 9$\times$ & 390 & 130 & 7.48 \\
Loukia & 14 & 13,503 & 67 & 3,793 & 57$\times$ & 420 & 140 & 3.11 \\
MUUFL & 11 & 53,687 & 183 & 23,246 & 127$\times$ & 330 & 110 & 0.61 \\
Nili Fossae & 9 & 26,710 & 228 & 8,563 & 38$\times$ & 270 & 90 & 1.01 \\
Pavia Centre & 9 & 148,152 & 2,685 & 65,971 & 25$\times$ & 270 & 90 & 0.18 \\
Pavia University & 9 & 42,776 & 947 & 18,649 & 20$\times$ & 270 & 90 & 0.63 \\
Pingan & 10 & 1,140,937 & 8,108 & 578,113 & 71$\times$ & 300 & 100 & 0.03 \\
Qingyun & 6 & 954,893 & 9,767 & 278,150 & 28$\times$ & 180 & 60 & 0.02 \\
Salinas & 16 & 54,129 & 916 & 11,271 & 12$\times$ & 480 & 160 & 0.89 \\
Tangdaowan & 18 & 557,366 & 749 & 140,904 & 188$\times$ & 540 & 180 & 0.10 \\
Trento & 6 & 30,214 & 479 & 10,501 & 22$\times$ & 180 & 60 & 0.60 \\
Utopia & 9 & 17,338 & 202 & 6,774 & 34$\times$ & 270 & 90 & 1.56 \\
WHU-Hi-HanChuan & 16 & 257,530 & 1,136 & 75,401 & 66$\times$ & 480 & 160 & 0.19 \\
WHU-Hi-HongHu & 22 & 386,693 & 1,002 & 163,285 & 163$\times$ & 660 & 220 & 0.17 \\
WHU-Hi-LongKou & 9 & 204,542 & 3,031 & 67,056 & 22$\times$ & 270 & 90 & 0.13 \\
\bottomrule
\end{tabular}
\end{table}


==> table/tab_perscene_a.tex <==
\begin{table}[p]
\centering
\caption{Per-model results on Indian Pines and Pavia University, under the protocol of \Cref{tab:protocol}. Each entry is the mean over five seeded runs with its sample standard deviation; the best value in each column is in bold. These two AVIRIS and ROSIS scenes are the most widely reported in the literature and are included so that results here can be read against published numbers.}
\label{tab:perscene_a}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
& \multicolumn{3}{c}{Indian Pines} & \multicolumn{3}{c}{Pavia University} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
Model & OA & AA & $\kappa$ & OA & AA & $\kappa$ \\
\midrule
\multicolumn{7}{@{}l}{\textit{CNN}} \\[1pt]
\quad \texttt{DKDMN} & 84.82\,\tiny{$\pm$\,1.84} & 91.64\,\tiny{$\pm$\,1.07} & 82.75\,\tiny{$\pm$\,2.09} & 95.44\,\tiny{$\pm$\,1.23} & 95.82\,\tiny{$\pm$\,1.73} & 94.08\,\tiny{$\pm$\,1.58} \\
\quad \texttt{SSRN} & 84.71\,\tiny{$\pm$\,3.92} & \textbf{91.99\,\tiny{$\pm$\,1.37}} & 82.66\,\tiny{$\pm$\,4.38} & \textbf{97.81\,\tiny{$\pm$\,0.52}} & \textbf{98.09\,\tiny{$\pm$\,0.38}} & \textbf{97.15\,\tiny{$\pm$\,0.66}} \\
\quad \texttt{FETNet} & 80.84\,\tiny{$\pm$\,1.27} & 89.29\,\tiny{$\pm$\,0.61} & 78.26\,\tiny{$\pm$\,1.45} & 87.36\,\tiny{$\pm$\,3.86} & 90.30\,\tiny{$\pm$\,1.85} & 83.93\,\tiny{$\pm$\,4.64} \\
\quad \texttt{ENL\_FCN} & 80.73\,\tiny{$\pm$\,2.17} & 90.37\,\tiny{$\pm$\,1.31} & 78.28\,\tiny{$\pm$\,2.41} & 94.43\,\tiny{$\pm$\,1.70} & 95.32\,\tiny{$\pm$\,0.58} & 92.81\,\tiny{$\pm$\,2.16} \\
\quad \texttt{DBDA} & 80.73\,\tiny{$\pm$\,3.85} & 89.34\,\tiny{$\pm$\,1.74} & 78.16\,\tiny{$\pm$\,4.29} & 97.46\,\tiny{$\pm$\,0.26} & 97.29\,\tiny{$\pm$\,0.46} & 96.69\,\tiny{$\pm$\,0.34} \\
\quad \texttt{SSTN} & 73.10\,\tiny{$\pm$\,4.64} & 84.54\,\tiny{$\pm$\,4.89} & 69.79\,\tiny{$\pm$\,5.32} & 94.18\,\tiny{$\pm$\,1.27} & 94.79\,\tiny{$\pm$\,0.68} & 92.47\,\tiny{$\pm$\,1.62} \\
\quad \texttt{SACNet} & 70.06\,\tiny{$\pm$\,3.50} & 80.54\,\tiny{$\pm$\,2.51} & 66.16\,\tiny{$\pm$\,3.93} & 91.93\,\tiny{$\pm$\,1.28} & 92.76\,\tiny{$\pm$\,1.26} & 89.56\,\tiny{$\pm$\,1.62} \\
\quad \texttt{S3ANet} & 69.59\,\tiny{$\pm$\,2.09} & 80.61\,\tiny{$\pm$\,1.92} & 65.71\,\tiny{$\pm$\,2.33} & 92.23\,\tiny{$\pm$\,1.47} & 92.83\,\tiny{$\pm$\,0.48} & 89.94\,\tiny{$\pm$\,1.85} \\
\quad \texttt{HybridSN} & 68.83\,\tiny{$\pm$\,2.05} & 80.85\,\tiny{$\pm$\,0.56} & 64.89\,\tiny{$\pm$\,2.07} & 90.73\,\tiny{$\pm$\,4.23} & 92.16\,\tiny{$\pm$\,1.51} & 88.09\,\tiny{$\pm$\,5.28} \\
\quad \texttt{pResNet} & 66.82\,\tiny{$\pm$\,8.43} & 79.77\,\tiny{$\pm$\,4.86} & 62.30\,\tiny{$\pm$\,9.38} & 94.10\,\tiny{$\pm$\,3.84} & 95.20\,\tiny{$\pm$\,0.55} & 92.44\,\tiny{$\pm$\,4.78} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Transformer}} \\[1pt]
\quad \texttt{CTMixer} & \textbf{84.91\,\tiny{$\pm$\,1.94}} & 91.74\,\tiny{$\pm$\,1.32} & \textbf{82.86\,\tiny{$\pm$\,2.20}} & 97.07\,\tiny{$\pm$\,0.27} & 97.07\,\tiny{$\pm$\,0.46} & 96.19\,\tiny{$\pm$\,0.35} \\
\quad \texttt{MVAHN} & 82.71\,\tiny{$\pm$\,5.41} & 90.76\,\tiny{$\pm$\,2.48} & 80.45\,\tiny{$\pm$\,6.03} & 97.57\,\tiny{$\pm$\,0.50} & 96.88\,\tiny{$\pm$\,0.86} & 96.83\,\tiny{$\pm$\,0.64} \\
\quad \texttt{GAHT} & 82.14\,\tiny{$\pm$\,1.64} & 90.30\,\tiny{$\pm$\,1.44} & 79.78\,\tiny{$\pm$\,1.84} & 91.77\,\tiny{$\pm$\,2.77} & 94.34\,\tiny{$\pm$\,0.86} & 89.47\,\tiny{$\pm$\,3.42} \\
\quad \texttt{3DConvSST} & 81.79\,\tiny{$\pm$\,3.53} & 90.50\,\tiny{$\pm$\,1.54} & 79.41\,\tiny{$\pm$\,3.94} & 96.05\,\tiny{$\pm$\,2.82} & 96.66\,\tiny{$\pm$\,1.73} & 94.89\,\tiny{$\pm$\,3.62} \\
\quad \texttt{SSFTTNet} & 81.30\,\tiny{$\pm$\,3.11} & 89.47\,\tiny{$\pm$\,2.29} & 78.82\,\tiny{$\pm$\,3.52} & 95.23\,\tiny{$\pm$\,1.86} & 96.03\,\tiny{$\pm$\,1.24} & 93.83\,\tiny{$\pm$\,2.37} \\
\quad \texttt{DSFormer} & 80.50\,\tiny{$\pm$\,2.79} & 88.82\,\tiny{$\pm$\,0.85} & 77.92\,\tiny{$\pm$\,3.11} & 96.50\,\tiny{$\pm$\,2.13} & 97.53\,\tiny{$\pm$\,0.59} & 95.47\,\tiny{$\pm$\,2.73} \\
\quad \texttt{MASSFormer} & 80.27\,\tiny{$\pm$\,2.73} & 89.37\,\tiny{$\pm$\,1.84} & 77.71\,\tiny{$\pm$\,3.05} & 92.53\,\tiny{$\pm$\,3.82} & 94.29\,\tiny{$\pm$\,2.55} & 90.40\,\tiny{$\pm$\,4.84} \\
\quad \texttt{MMFormer} & 80.15\,\tiny{$\pm$\,4.49} & 88.25\,\tiny{$\pm$\,2.86} & 77.47\,\tiny{$\pm$\,5.02} & 94.44\,\tiny{$\pm$\,3.21} & 95.81\,\tiny{$\pm$\,1.64} & 92.86\,\tiny{$\pm$\,4.06} \\
\quad \texttt{MorphFormer} & 79.46\,\tiny{$\pm$\,3.62} & 88.77\,\tiny{$\pm$\,2.11} & 76.79\,\tiny{$\pm$\,4.06} & 96.82\,\tiny{$\pm$\,0.41} & 96.63\,\tiny{$\pm$\,0.36} & 95.87\,\tiny{$\pm$\,0.53} \\
\quad \texttt{FAHM} & 76.08\,\tiny{$\pm$\,5.97} & 86.52\,\tiny{$\pm$\,3.61} & 72.95\,\tiny{$\pm$\,6.57} & 97.15\,\tiny{$\pm$\,0.53} & 96.21\,\tiny{$\pm$\,0.97} & 96.28\,\tiny{$\pm$\,0.69} \\
\quad \texttt{SpectralFormer} & 74.18\,\tiny{$\pm$\,2.77} & 85.05\,\tiny{$\pm$\,2.51} & 70.93\,\tiny{$\pm$\,3.04} & 91.69\,\tiny{$\pm$\,0.76} & 90.71\,\tiny{$\pm$\,0.70} & 89.15\,\tiny{$\pm$\,1.01} \\
\quad \texttt{MFT} & 72.08\,\tiny{$\pm$\,3.87} & 83.65\,\tiny{$\pm$\,3.55} & 68.52\,\tiny{$\pm$\,4.46} & 95.59\,\tiny{$\pm$\,1.18} & 95.52\,\tiny{$\pm$\,1.06} & 94.27\,\tiny{$\pm$\,1.53} \\
\quad \texttt{HSIC\_SClusterFormer} & 70.28\,\tiny{$\pm$\,3.33} & 81.58\,\tiny{$\pm$\,3.28} & 66.41\,\tiny{$\pm$\,3.32} & 90.36\,\tiny{$\pm$\,1.38} & 92.74\,\tiny{$\pm$\,3.50} & 87.72\,\tiny{$\pm$\,1.78} \\
\quad \texttt{S2Gformer} & 61.71\,\tiny{$\pm$\,1.94} & 77.32\,\tiny{$\pm$\,1.20} & 57.02\,\tiny{$\pm$\,2.23} & 74.53\,\tiny{$\pm$\,7.44} & 82.39\,\tiny{$\pm$\,2.88} & 68.48\,\tiny{$\pm$\,8.21} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Mamba / SSM}} \\[1pt]
\quad \texttt{MambaLG} & 82.47\,\tiny{$\pm$\,3.96} & 90.24\,\tiny{$\pm$\,1.11} & 80.17\,\tiny{$\pm$\,4.34} & 97.21\,\tiny{$\pm$\,0.96} & 96.79\,\tiny{$\pm$\,0.60} & 96.35\,\tiny{$\pm$\,1.24} \\
\quad \texttt{IGroupSS-Mamba} & 81.08\,\tiny{$\pm$\,0.87} & 90.35\,\tiny{$\pm$\,0.88} & 78.65\,\tiny{$\pm$\,1.00} & 97.12\,\tiny{$\pm$\,0.73} & 97.65\,\tiny{$\pm$\,0.35} & 96.26\,\tiny{$\pm$\,0.93} \\
\quad \texttt{S2Mamba} & 78.12\,\tiny{$\pm$\,3.46} & 88.10\,\tiny{$\pm$\,0.95} & 75.35\,\tiny{$\pm$\,3.79} & 97.04\,\tiny{$\pm$\,0.66} & 97.63\,\tiny{$\pm$\,0.17} & 96.15\,\tiny{$\pm$\,0.84} \\
\quad \texttt{HyperMamba} & 77.69\,\tiny{$\pm$\,1.59} & 87.59\,\tiny{$\pm$\,2.09} & 74.77\,\tiny{$\pm$\,1.90} & 94.96\,\tiny{$\pm$\,0.98} & 95.84\,\tiny{$\pm$\,1.28} & 93.44\,\tiny{$\pm$\,1.27} \\
\quad \texttt{MambaHSI\_Plus} & 77.18\,\tiny{$\pm$\,4.16} & 87.55\,\tiny{$\pm$\,1.77} & 74.33\,\tiny{$\pm$\,4.52} & 94.25\,\tiny{$\pm$\,0.86} & 94.67\,\tiny{$\pm$\,1.03} & 92.53\,\tiny{$\pm$\,1.11} \\
\quad \texttt{PHDMamba} & 76.86\,\tiny{$\pm$\,3.24} & 87.38\,\tiny{$\pm$\,1.94} & 73.88\,\tiny{$\pm$\,3.60} & 95.33\,\tiny{$\pm$\,0.76} & 96.42\,\tiny{$\pm$\,0.59} & 93.95\,\tiny{$\pm$\,0.94} \\
\quad \texttt{MiM} & 76.83\,\tiny{$\pm$\,9.31} & 87.56\,\tiny{$\pm$\,4.77} & 74.06\,\tiny{$\pm$\,10.15} & 96.57\,\tiny{$\pm$\,0.97} & 97.21\,\tiny{$\pm$\,0.28} & 95.55\,\tiny{$\pm$\,1.24} \\
\quad \texttt{MLFMamba} & 76.62\,\tiny{$\pm$\,5.18} & 86.91\,\tiny{$\pm$\,2.11} & 73.70\,\tiny{$\pm$\,5.66} & 86.16\,\tiny{$\pm$\,4.68} & 90.34\,\tiny{$\pm$\,0.92} & 82.59\,\tiny{$\pm$\,5.49} \\
\quad \texttt{MambaHSI} & 76.18\,\tiny{$\pm$\,2.77} & 86.22\,\tiny{$\pm$\,1.11} & 73.19\,\tiny{$\pm$\,3.06} & 92.62\,\tiny{$\pm$\,1.97} & 93.77\,\tiny{$\pm$\,1.01} & 90.49\,\tiny{$\pm$\,2.51} \\
\quad \texttt{MambaMoE} & 75.89\,\tiny{$\pm$\,1.45} & 86.36\,\tiny{$\pm$\,1.62} & 72.81\,\tiny{$\pm$\,1.62} & 94.43\,\tiny{$\pm$\,0.49} & 95.36\,\tiny{$\pm$\,0.95} & 92.78\,\tiny{$\pm$\,0.65} \\
\quad \texttt{HyPyraMamba} & 73.72\,\tiny{$\pm$\,2.77} & 84.88\,\tiny{$\pm$\,1.86} & 70.41\,\tiny{$\pm$\,2.89} & 93.11\,\tiny{$\pm$\,1.40} & 93.89\,\tiny{$\pm$\,0.70} & 91.08\,\tiny{$\pm$\,1.80} \\
\quad \texttt{EMamba} & 73.54\,\tiny{$\pm$\,2.01} & 86.28\,\tiny{$\pm$\,1.64} & 70.26\,\tiny{$\pm$\,2.29} & 95.78\,\tiny{$\pm$\,0.95} & 96.56\,\tiny{$\pm$\,0.34} & 94.52\,\tiny{$\pm$\,1.20} \\
\quad \texttt{FuzzySpectralMamba} & 73.23\,\tiny{$\pm$\,3.56} & 85.20\,\tiny{$\pm$\,2.25} & 69.86\,\tiny{$\pm$\,3.99} & 95.74\,\tiny{$\pm$\,1.61} & 96.63\,\tiny{$\pm$\,0.38} & 94.48\,\tiny{$\pm$\,2.05} \\
\quad \texttt{MorpMamba} & 64.30\,\tiny{$\pm$\,1.49} & 78.07\,\tiny{$\pm$\,0.95} & 60.03\,\tiny{$\pm$\,1.55} & 88.97\,\tiny{$\pm$\,3.97} & 90.11\,\tiny{$\pm$\,2.39} & 85.84\,\tiny{$\pm$\,4.92} \\
\quad \texttt{SSMamba} & 63.12\,\tiny{$\pm$\,8.27} & 77.15\,\tiny{$\pm$\,5.75} & 58.59\,\tiny{$\pm$\,9.06} & 85.58\,\tiny{$\pm$\,8.13} & 90.04\,\tiny{$\pm$\,3.46} & 81.89\,\tiny{$\pm$\,9.75} \\
\quad \texttt{MHSSMamba} & 59.66\,\tiny{$\pm$\,7.47} & 72.77\,\tiny{$\pm$\,7.06} & 54.79\,\tiny{$\pm$\,8.46} & 76.71\,\tiny{$\pm$\,2.19} & 78.58\,\tiny{$\pm$\,0.65} & 70.36\,\tiny{$\pm$\,2.48} \\
\quad \texttt{ConvVitMamba} & 52.39\,\tiny{$\pm$\,4.05} & 67.47\,\tiny{$\pm$\,4.28} & 46.44\,\tiny{$\pm$\,4.29} & 77.59\,\tiny{$\pm$\,22.53} & 83.49\,\tiny{$\pm$\,9.48} & 73.30\,\tiny{$\pm$\,25.25} \\
\quad \texttt{WaveMamba} & 31.98\,\tiny{$\pm$\,4.07} & 27.02\,\tiny{$\pm$\,4.05} & 23.43\,\tiny{$\pm$\,2.66} & 48.05\,\tiny{$\pm$\,10.67} & 39.64\,\tiny{$\pm$\,10.62} & 33.07\,\tiny{$\pm$\,10.92} \\
\quad \texttt{GraphMamba} & 26.60\,\tiny{$\pm$\,40.07} & 31.53\,\tiny{$\pm$\,43.79} & 22.63\,\tiny{$\pm$\,39.39} & 94.87\,\tiny{$\pm$\,4.11} & 96.11\,\tiny{$\pm$\,1.59} & 93.40\,\tiny{$\pm$\,5.20} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Graph / GCN}} \\[1pt]
\quad \texttt{MS2GCAN} & 84.15\,\tiny{$\pm$\,7.49} & 91.08\,\tiny{$\pm$\,4.35} & 82.00\,\tiny{$\pm$\,8.40} & 94.23\,\tiny{$\pm$\,3.34} & 93.09\,\tiny{$\pm$\,4.87} & 92.55\,\tiny{$\pm$\,4.24} \\
\quad \texttt{GTCFN} & 77.68\,\tiny{$\pm$\,2.82} & 88.28\,\tiny{$\pm$\,1.59} & 74.88\,\tiny{$\pm$\,3.11} & 96.74\,\tiny{$\pm$\,1.16} & 96.61\,\tiny{$\pm$\,1.02} & 95.76\,\tiny{$\pm$\,1.50} \\
\quad \texttt{MCTGCL} & 72.32\,\tiny{$\pm$\,6.12} & 85.63\,\tiny{$\pm$\,2.90} & 69.11\,\tiny{$\pm$\,6.65} & 87.27\,\tiny{$\pm$\,3.40} & 91.47\,\tiny{$\pm$\,3.64} & 83.86\,\tiny{$\pm$\,4.19} \\
\quad \texttt{GraphGST} & 71.48\,\tiny{$\pm$\,4.15} & 85.26\,\tiny{$\pm$\,1.36} & 68.21\,\tiny{$\pm$\,4.33} & 91.70\,\tiny{$\pm$\,2.20} & 91.60\,\tiny{$\pm$\,2.88} & 89.30\,\tiny{$\pm$\,2.80} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{KAN}} \\[1pt]
\quad \texttt{HyperKAN} & 79.00\,\tiny{$\pm$\,3.04} & 88.76\,\tiny{$\pm$\,1.49} & 76.25\,\tiny{$\pm$\,3.39} & 96.15\,\tiny{$\pm$\,1.05} & 96.37\,\tiny{$\pm$\,0.99} & 94.99\,\tiny{$\pm$\,1.36} \\
\quad \texttt{HSIConvKAN} & 59.65\,\tiny{$\pm$\,5.49} & 74.89\,\tiny{$\pm$\,2.61} & 54.74\,\tiny{$\pm$\,5.94} & 86.48\,\tiny{$\pm$\,2.39} & 87.33\,\tiny{$\pm$\,1.13} & 82.63\,\tiny{$\pm$\,2.94} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Self-supervised}} \\[1pt]
\quad \texttt{HSIMAE} & 65.81\,\tiny{$\pm$\,2.37} & 79.96\,\tiny{$\pm$\,1.58} & 61.86\,\tiny{$\pm$\,2.34} & 84.04\,\tiny{$\pm$\,3.59} & 86.67\,\tiny{$\pm$\,2.77} & 79.50\,\tiny{$\pm$\,4.53} \\
\quad \texttt{LFSMIM} & 60.20\,\tiny{$\pm$\,3.24} & 74.54\,\tiny{$\pm$\,1.34} & 55.58\,\tiny{$\pm$\,3.20} & 87.86\,\tiny{$\pm$\,4.08} & 88.71\,\tiny{$\pm$\,3.05} & 84.37\,\tiny{$\pm$\,5.16} \\
\quad \texttt{HSIC\_FM} & 31.93\,\tiny{$\pm$\,25.30} & 47.35\,\tiny{$\pm$\,27.16} & 27.20\,\tiny{$\pm$\,23.72} & 70.28\,\tiny{$\pm$\,7.60} & 72.50\,\tiny{$\pm$\,4.49} & 62.47\,\tiny{$\pm$\,8.64} \\
\addlinespace[2pt]
\bottomrule
\end{tabular}
\end{table}


==> table/tab_perscene_b.tex <==
\begin{table}[p]
\centering
\caption{Per-model results on WHU Hi LongKou and Nili Fossae, under the protocol of \Cref{tab:protocol}. Each entry is the mean over five seeded runs with its sample standard deviation; the best value in each column is in bold. A UAV agricultural mosaic and a Mars CRISM scene, included to show behaviour outside the classical benchmarks.}
\label{tab:perscene_b}
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
& \multicolumn{3}{c}{WHU Hi LongKou} & \multicolumn{3}{c}{Nili Fossae} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
Model & OA & AA & $\kappa$ & OA & AA & $\kappa$ \\
\midrule
\multicolumn{7}{@{}l}{\textit{CNN}} \\[1pt]
\quad \texttt{SSRN} & 98.36\,\tiny{$\pm$\,0.33} & 97.44\,\tiny{$\pm$\,0.43} & 97.85\,\tiny{$\pm$\,0.43} & 96.69\,\tiny{$\pm$\,1.03} & 95.29\,\tiny{$\pm$\,1.77} & 95.77\,\tiny{$\pm$\,1.31} \\
\quad \texttt{DBDA} & 98.05\,\tiny{$\pm$\,0.17} & 96.78\,\tiny{$\pm$\,0.25} & 97.45\,\tiny{$\pm$\,0.22} & 96.45\,\tiny{$\pm$\,0.54} & 95.76\,\tiny{$\pm$\,0.67} & 95.47\,\tiny{$\pm$\,0.69} \\
\quad \texttt{pResNet} & 97.73\,\tiny{$\pm$\,1.23} & 97.15\,\tiny{$\pm$\,1.60} & 97.03\,\tiny{$\pm$\,1.61} & 97.06\,\tiny{$\pm$\,0.57} & 95.90\,\tiny{$\pm$\,1.06} & 96.23\,\tiny{$\pm$\,0.73} \\
\quad \texttt{DKDMN} & 97.64\,\tiny{$\pm$\,0.54} & 95.90\,\tiny{$\pm$\,0.80} & 96.91\,\tiny{$\pm$\,0.70} & 93.73\,\tiny{$\pm$\,1.45} & 94.46\,\tiny{$\pm$\,0.86} & 92.01\,\tiny{$\pm$\,1.85} \\
\quad \texttt{FETNet} & 97.31\,\tiny{$\pm$\,0.86} & 97.14\,\tiny{$\pm$\,0.43} & 96.50\,\tiny{$\pm$\,1.11} & 96.19\,\tiny{$\pm$\,1.44} & 94.03\,\tiny{$\pm$\,2.22} & 95.11\,\tiny{$\pm$\,1.85} \\
\quad \texttt{SSTN} & 97.20\,\tiny{$\pm$\,0.34} & 95.33\,\tiny{$\pm$\,0.45} & 96.32\,\tiny{$\pm$\,0.44} & 96.11\,\tiny{$\pm$\,0.42} & 95.21\,\tiny{$\pm$\,0.72} & 95.04\,\tiny{$\pm$\,0.54} \\
\quad \texttt{SACNet} & 97.00\,\tiny{$\pm$\,0.17} & 95.35\,\tiny{$\pm$\,0.40} & 96.07\,\tiny{$\pm$\,0.21} & 95.10\,\tiny{$\pm$\,1.36} & 95.66\,\tiny{$\pm$\,0.27} & 93.77\,\tiny{$\pm$\,1.72} \\
\quad \texttt{ENL\_FCN} & 96.93\,\tiny{$\pm$\,0.60} & 95.58\,\tiny{$\pm$\,1.37} & 95.99\,\tiny{$\pm$\,0.78} & 92.22\,\tiny{$\pm$\,3.61} & 93.26\,\tiny{$\pm$\,2.41} & 90.12\,\tiny{$\pm$\,4.47} \\
\quad \texttt{S3ANet} & 96.82\,\tiny{$\pm$\,0.46} & 96.33\,\tiny{$\pm$\,0.30} & 95.85\,\tiny{$\pm$\,0.60} & 96.94\,\tiny{$\pm$\,1.34} & 97.01\,\tiny{$\pm$\,0.77} & 96.09\,\tiny{$\pm$\,1.70} \\
\quad \texttt{HybridSN} & 95.04\,\tiny{$\pm$\,0.86} & 93.00\,\tiny{$\pm$\,1.03} & 93.52\,\tiny{$\pm$\,1.11} & 95.11\,\tiny{$\pm$\,1.13} & 95.43\,\tiny{$\pm$\,1.15} & 93.76\,\tiny{$\pm$\,1.44} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Transformer}} \\[1pt]
\quad \texttt{MMFormer} & \textbf{98.84\,\tiny{$\pm$\,0.25}} & \textbf{98.41\,\tiny{$\pm$\,0.33}} & \textbf{98.47\,\tiny{$\pm$\,0.33}} & 97.36\,\tiny{$\pm$\,0.35} & 96.93\,\tiny{$\pm$\,0.48} & 96.63\,\tiny{$\pm$\,0.43} \\
\quad \texttt{FAHM} & 98.29\,\tiny{$\pm$\,0.50} & 97.67\,\tiny{$\pm$\,0.94} & 97.76\,\tiny{$\pm$\,0.66} & 96.42\,\tiny{$\pm$\,1.96} & 96.33\,\tiny{$\pm$\,1.41} & 95.43\,\tiny{$\pm$\,2.49} \\
\quad \texttt{DSFormer} & 98.20\,\tiny{$\pm$\,0.12} & 97.47\,\tiny{$\pm$\,0.95} & 97.64\,\tiny{$\pm$\,0.16} & 95.49\,\tiny{$\pm$\,2.28} & 95.36\,\tiny{$\pm$\,1.38} & 94.26\,\tiny{$\pm$\,2.88} \\
\quad \texttt{MVAHN} & 98.17\,\tiny{$\pm$\,0.64} & 96.83\,\tiny{$\pm$\,1.17} & 97.60\,\tiny{$\pm$\,0.83} & 97.48\,\tiny{$\pm$\,0.81} & 96.58\,\tiny{$\pm$\,0.68} & 96.78\,\tiny{$\pm$\,1.04} \\
\quad \texttt{MASSFormer} & 97.87\,\tiny{$\pm$\,0.41} & 97.46\,\tiny{$\pm$\,0.64} & 97.21\,\tiny{$\pm$\,0.53} & 97.31\,\tiny{$\pm$\,0.46} & 96.64\,\tiny{$\pm$\,0.89} & 96.56\,\tiny{$\pm$\,0.59} \\
\quad \texttt{SSFTTNet} & 97.46\,\tiny{$\pm$\,0.99} & 97.00\,\tiny{$\pm$\,1.31} & 96.68\,\tiny{$\pm$\,1.28} & 96.68\,\tiny{$\pm$\,0.84} & 96.62\,\tiny{$\pm$\,1.29} & 95.76\,\tiny{$\pm$\,1.07} \\
\quad \texttt{3DConvSST} & 97.45\,\tiny{$\pm$\,0.71} & 96.43\,\tiny{$\pm$\,0.10} & 96.66\,\tiny{$\pm$\,0.92} & 96.19\,\tiny{$\pm$\,0.77} & 95.83\,\tiny{$\pm$\,0.94} & 95.13\,\tiny{$\pm$\,0.99} \\
\quad \texttt{MorphFormer} & 97.27\,\tiny{$\pm$\,0.15} & 96.50\,\tiny{$\pm$\,0.26} & 96.42\,\tiny{$\pm$\,0.20} & 95.74\,\tiny{$\pm$\,1.02} & 95.56\,\tiny{$\pm$\,0.68} & 94.57\,\tiny{$\pm$\,1.29} \\
\quad \texttt{SpectralFormer} & 97.16\,\tiny{$\pm$\,0.80} & 95.01\,\tiny{$\pm$\,2.12} & 96.27\,\tiny{$\pm$\,1.05} & 96.24\,\tiny{$\pm$\,1.17} & 95.50\,\tiny{$\pm$\,0.70} & 95.19\,\tiny{$\pm$\,1.49} \\
\quad \texttt{CTMixer} & 96.63\,\tiny{$\pm$\,0.37} & 96.91\,\tiny{$\pm$\,0.20} & 95.61\,\tiny{$\pm$\,0.48} & 92.58\,\tiny{$\pm$\,0.63} & 93.40\,\tiny{$\pm$\,0.40} & 90.56\,\tiny{$\pm$\,0.80} \\
\quad \texttt{MFT} & 96.33\,\tiny{$\pm$\,1.76} & 94.74\,\tiny{$\pm$\,1.97} & 95.19\,\tiny{$\pm$\,2.29} & 95.40\,\tiny{$\pm$\,1.64} & 94.93\,\tiny{$\pm$\,1.71} & 94.12\,\tiny{$\pm$\,2.10} \\
\quad \texttt{S2Gformer} & 95.86\,\tiny{$\pm$\,0.70} & 93.66\,\tiny{$\pm$\,2.42} & 94.59\,\tiny{$\pm$\,0.91} & 96.17\,\tiny{$\pm$\,1.20} & 94.70\,\tiny{$\pm$\,1.23} & 95.11\,\tiny{$\pm$\,1.51} \\
\quad \texttt{HSIC\_SClusterFormer} & 94.11\,\tiny{$\pm$\,1.67} & 93.27\,\tiny{$\pm$\,1.24} & 92.35\,\tiny{$\pm$\,2.13} & 93.91\,\tiny{$\pm$\,3.89} & 92.62\,\tiny{$\pm$\,5.03} & 92.28\,\tiny{$\pm$\,4.88} \\
\quad \texttt{GAHT} & 92.62\,\tiny{$\pm$\,6.17} & 93.89\,\tiny{$\pm$\,2.97} & 90.60\,\tiny{$\pm$\,7.65} & 88.88\,\tiny{$\pm$\,0.88} & 90.01\,\tiny{$\pm$\,1.36} & 85.91\,\tiny{$\pm$\,1.14} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Mamba / SSM}} \\[1pt]
\quad \texttt{IGroupSS-Mamba} & 98.27\,\tiny{$\pm$\,0.04} & 98.26\,\tiny{$\pm$\,0.15} & 97.73\,\tiny{$\pm$\,0.05} & 96.92\,\tiny{$\pm$\,0.47} & 96.72\,\tiny{$\pm$\,0.44} & 96.08\,\tiny{$\pm$\,0.60} \\
\quad \texttt{S2Mamba} & 98.25\,\tiny{$\pm$\,0.10} & 97.94\,\tiny{$\pm$\,0.92} & 97.71\,\tiny{$\pm$\,0.14} & 97.71\,\tiny{$\pm$\,0.67} & 97.09\,\tiny{$\pm$\,0.81} & 97.07\,\tiny{$\pm$\,0.86} \\
\quad \texttt{MambaHSI\_Plus} & 98.13\,\tiny{$\pm$\,0.45} & 97.38\,\tiny{$\pm$\,0.60} & 97.55\,\tiny{$\pm$\,0.59} & 96.40\,\tiny{$\pm$\,2.34} & 96.18\,\tiny{$\pm$\,1.64} & 95.41\,\tiny{$\pm$\,2.98} \\
\quad \texttt{PHDMamba} & 97.93\,\tiny{$\pm$\,0.61} & 97.45\,\tiny{$\pm$\,1.08} & 97.29\,\tiny{$\pm$\,0.81} & 96.52\,\tiny{$\pm$\,1.11} & 96.40\,\tiny{$\pm$\,0.74} & 95.56\,\tiny{$\pm$\,1.42} \\
\quad \texttt{MambaHSI} & 97.87\,\tiny{$\pm$\,0.18} & 96.94\,\tiny{$\pm$\,0.68} & 97.20\,\tiny{$\pm$\,0.24} & 95.23\,\tiny{$\pm$\,1.20} & 94.47\,\tiny{$\pm$\,1.90} & 93.91\,\tiny{$\pm$\,1.52} \\
\quad \texttt{MLFMamba} & 97.86\,\tiny{$\pm$\,0.16} & 96.94\,\tiny{$\pm$\,0.87} & 97.19\,\tiny{$\pm$\,0.21} & 96.68\,\tiny{$\pm$\,0.94} & 96.24\,\tiny{$\pm$\,0.70} & 95.77\,\tiny{$\pm$\,1.20} \\
\quad \texttt{MambaMoE} & 97.70\,\tiny{$\pm$\,0.21} & 97.25\,\tiny{$\pm$\,0.88} & 96.98\,\tiny{$\pm$\,0.27} & 95.98\,\tiny{$\pm$\,1.64} & 96.09\,\tiny{$\pm$\,1.49} & 94.88\,\tiny{$\pm$\,2.07} \\
\quad \texttt{MambaLG} & 97.60\,\tiny{$\pm$\,0.60} & 97.24\,\tiny{$\pm$\,1.08} & 96.87\,\tiny{$\pm$\,0.78} & 97.53\,\tiny{$\pm$\,0.28} & 96.64\,\tiny{$\pm$\,0.61} & 96.84\,\tiny{$\pm$\,0.37} \\
\quad \texttt{HyperMamba} & 97.25\,\tiny{$\pm$\,0.36} & 97.60\,\tiny{$\pm$\,0.40} & 96.41\,\tiny{$\pm$\,0.46} & \textbf{97.83\,\tiny{$\pm$\,0.31}} & \textbf{97.58\,\tiny{$\pm$\,0.49}} & \textbf{97.23\,\tiny{$\pm$\,0.39}} \\
\quad \texttt{SSMamba} & 97.07\,\tiny{$\pm$\,1.01} & 97.57\,\tiny{$\pm$\,0.45} & 96.18\,\tiny{$\pm$\,1.31} & 92.74\,\tiny{$\pm$\,4.07} & 93.21\,\tiny{$\pm$\,2.26} & 90.79\,\tiny{$\pm$\,5.09} \\
\quad \texttt{MiM} & 97.07\,\tiny{$\pm$\,1.02} & 95.98\,\tiny{$\pm$\,1.61} & 96.17\,\tiny{$\pm$\,1.34} & 93.49\,\tiny{$\pm$\,1.40} & 92.54\,\tiny{$\pm$\,1.94} & 91.73\,\tiny{$\pm$\,1.77} \\
\quad \texttt{EMamba} & 97.01\,\tiny{$\pm$\,0.50} & 96.72\,\tiny{$\pm$\,0.23} & 96.09\,\tiny{$\pm$\,0.65} & 95.33\,\tiny{$\pm$\,0.34} & 94.35\,\tiny{$\pm$\,0.46} & 94.04\,\tiny{$\pm$\,0.44} \\
\quad \texttt{GraphMamba} & 96.88\,\tiny{$\pm$\,1.53} & 97.14\,\tiny{$\pm$\,0.61} & 95.93\,\tiny{$\pm$\,1.97} & 96.32\,\tiny{$\pm$\,0.94} & 93.95\,\tiny{$\pm$\,4.24} & 95.29\,\tiny{$\pm$\,1.22} \\
\quad \texttt{HyPyraMamba} & 96.84\,\tiny{$\pm$\,1.33} & 96.53\,\tiny{$\pm$\,1.55} & 95.88\,\tiny{$\pm$\,1.72} & 97.04\,\tiny{$\pm$\,0.69} & 95.96\,\tiny{$\pm$\,0.59} & 96.22\,\tiny{$\pm$\,0.88} \\
\quad \texttt{FuzzySpectralMamba} & 96.72\,\tiny{$\pm$\,1.15} & 95.71\,\tiny{$\pm$\,1.06} & 95.71\,\tiny{$\pm$\,1.49} & 94.85\,\tiny{$\pm$\,0.54} & 93.43\,\tiny{$\pm$\,0.18} & 93.45\,\tiny{$\pm$\,0.68} \\
\quad \texttt{MorpMamba} & 95.51\,\tiny{$\pm$\,0.40} & 94.68\,\tiny{$\pm$\,0.70} & 94.14\,\tiny{$\pm$\,0.52} & 93.06\,\tiny{$\pm$\,0.70} & 93.87\,\tiny{$\pm$\,0.69} & 91.19\,\tiny{$\pm$\,0.88} \\
\quad \texttt{MHSSMamba} & 91.39\,\tiny{$\pm$\,4.31} & 84.28\,\tiny{$\pm$\,7.22} & 88.79\,\tiny{$\pm$\,5.60} & 94.49\,\tiny{$\pm$\,1.67} & 93.05\,\tiny{$\pm$\,1.71} & 92.98\,\tiny{$\pm$\,2.10} \\
\quad \texttt{ConvVitMamba} & 86.75\,\tiny{$\pm$\,12.13} & 84.89\,\tiny{$\pm$\,10.36} & 83.49\,\tiny{$\pm$\,14.51} & 95.41\,\tiny{$\pm$\,1.15} & 93.78\,\tiny{$\pm$\,1.94} & 94.14\,\tiny{$\pm$\,1.46} \\
\quad \texttt{WaveMamba} & 74.53\,\tiny{$\pm$\,10.24} & 67.45\,\tiny{$\pm$\,3.33} & 68.66\,\tiny{$\pm$\,11.66} & 80.02\,\tiny{$\pm$\,2.14} & 73.89\,\tiny{$\pm$\,3.65} & 74.79\,\tiny{$\pm$\,2.71} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Graph / GCN}} \\[1pt]
\quad \texttt{MS2GCAN} & 98.33\,\tiny{$\pm$\,1.08} & 98.36\,\tiny{$\pm$\,0.44} & 97.81\,\tiny{$\pm$\,1.41} & 96.88\,\tiny{$\pm$\,0.19} & 95.50\,\tiny{$\pm$\,1.58} & 96.01\,\tiny{$\pm$\,0.24} \\
\quad \texttt{MCTGCL} & 97.39\,\tiny{$\pm$\,0.53} & 96.52\,\tiny{$\pm$\,0.90} & 96.58\,\tiny{$\pm$\,0.69} & 95.46\,\tiny{$\pm$\,2.02} & 94.90\,\tiny{$\pm$\,1.84} & 94.21\,\tiny{$\pm$\,2.56} \\
\quad \texttt{GTCFN} & 97.35\,\tiny{$\pm$\,0.08} & 95.99\,\tiny{$\pm$\,0.98} & 96.53\,\tiny{$\pm$\,0.10} & 93.57\,\tiny{$\pm$\,1.16} & 94.17\,\tiny{$\pm$\,1.32} & 91.80\,\tiny{$\pm$\,1.50} \\
\quad \texttt{GraphGST} & 92.63\,\tiny{$\pm$\,4.48} & 91.50\,\tiny{$\pm$\,3.36} & 90.49\,\tiny{$\pm$\,5.67} & 89.33\,\tiny{$\pm$\,4.05} & 78.23\,\tiny{$\pm$\,5.20} & 86.31\,\tiny{$\pm$\,5.18} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{KAN}} \\[1pt]
\quad \texttt{HyperKAN} & 97.45\,\tiny{$\pm$\,0.35} & 97.72\,\tiny{$\pm$\,0.03} & 96.67\,\tiny{$\pm$\,0.45} & 94.38\,\tiny{$\pm$\,0.84} & 94.97\,\tiny{$\pm$\,0.93} & 92.86\,\tiny{$\pm$\,1.07} \\
\quad \texttt{HSIConvKAN} & 92.47\,\tiny{$\pm$\,1.24} & 92.12\,\tiny{$\pm$\,1.04} & 90.27\,\tiny{$\pm$\,1.57} & 86.31\,\tiny{$\pm$\,2.17} & 87.46\,\tiny{$\pm$\,1.72} & 82.81\,\tiny{$\pm$\,2.69} \\
\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textit{Self-supervised}} \\[1pt]
\quad \texttt{HSIMAE} & 95.84\,\tiny{$\pm$\,1.25} & 92.03\,\tiny{$\pm$\,4.13} & 94.57\,\tiny{$\pm$\,1.63} & 95.94\,\tiny{$\pm$\,0.59} & 95.50\,\tiny{$\pm$\,0.31} & 94.82\,\tiny{$\pm$\,0.75} \\
\quad \texttt{LFSMIM} & 95.02\,\tiny{$\pm$\,1.52} & 95.85\,\tiny{$\pm$\,0.55} & 93.53\,\tiny{$\pm$\,1.93} & 92.52\,\tiny{$\pm$\,2.01} & 92.69\,\tiny{$\pm$\,1.28} & 90.50\,\tiny{$\pm$\,2.52} \\
\quad \texttt{HSIC\_FM} & 78.98\,\tiny{$\pm$\,5.43} & 80.20\,\tiny{$\pm$\,6.49} & 73.63\,\tiny{$\pm$\,6.67} & 34.43\,\tiny{$\pm$\,10.57} & 21.41\,\tiny{$\pm$\,4.58} & 16.76\,\tiny{$\pm$\,12.00} \\
\addlinespace[2pt]
\bottomrule
\end{tabular}
\end{table}

